On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo

Riemannian manifold Hamiltonian Monte Carlo (RMHMC) is a sampling algorithm that seeks to adapt proposals to the local geometry of the posterior distribution. The specific form of the Hamiltonian used in RMHMC necessitates {\it implicitly-defined} numerical integrators in order to sustain reversibility and volume-preservation, two properties that are necessary to establish detailed balance of RMHMC. In practice, these implicit equations are solved to a non-zero convergence tolerance via fixed-point iteration. However, the effect of these convergence thresholds on the ergodicity and computational efficiency properties of RMHMC are not well understood. The purpose of this research is to elucidate these relationships through numerous case studies. Our analysis reveals circumstances wherein the RMHMC algorithm is sensitive, and insensitive, to these convergence tolerances. Our empirical analysis examines several aspects of the computation: (i) we examine the ergodicity of the RMHMC Markov chain by employing statistical methods for comparing probability measures based on collections of samples; (ii) we investigate the degree to which detailed balance is violated by measuring errors in reversibility and volume-preservation; (iii) we assess the efficiency of the RMHMC Markov chain in terms of time-normalized ESS. In each of these cases, we investigate the sensitivity of these metrics to the convergence threshold and further contextualize our results in terms of comparison against Euclidean HMC. We propose a method by which one may select the convergence tolerance within a Bayesian inference application using techniques of stochastic approximation and we examine Newton's method, an alternative to fixed point iterations, which can eliminate much of the sensitivity of RMHMC to the convergence threshold.

==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/algorithms/hamiltonian-monte-carlo.tex <==
\begin{algorithm}[t!]
  \caption{Pseudo-code implementing the Hamiltonian Monte Carlo (HMC) algorithm. Given an initial position, a random momentum is generated and a reversible, volume preserving integrator is applied to this location in phase space. A Metropolis-Hastings correction is then applied to the output of the integrator in order to ensure detailed balance. When the metric $\mathbf{G}$ is constant with respect to $q$, the resulting Hamiltonian is separable and the leapfrog integrator may be used; on the other hand, if $\mathbf{G}$ depends on position then the generalized leapfrog integrator should be used to ensure reversibility and volume preservation.}
  \label{alg:hamiltonian-monte-carlo}
  \begin{algorithmic}
    \STATE {\bf Input:} An initial state $q_n\in \R^m$ and momentum $p_n \in\R^m$, a smooth log-density
    $\mathcal{L}:\R^m\to\R$, a Riemannian metric $\mathbf{G}:\R^m\to\R^m\times\R^m$, a reversible and volume-preserving numerical integrator $\Phi_\epsilon^k : \R^m\times\R^m\to\R^m\times\R^m$ consisting of $k\in\mathbb{N}$ steps with step-size $\epsilon\in \R$.
    \STATE Define the function
    \begin{align}
      H(q, p) = -\mathcal{L}(q) + \frac{1}{2} \log \mathrm{det}(\mathbf{G}(q)) + \frac{1}{2} p^\top\mathbf{G}(q)^{-1}p.
    \end{align}
    \STATE Apply the numerical integrator to obtain the proposal state for the Markov chain $(\tilde{q}_{n+1}, \hat{p}_{n+1}) = \Phi_\epsilon^k(q_n, p_n)$.
    \STATE Apply the momentum flip operator to produce a self-inverse proposal $\tilde{p}_{n+1} = -\hat{p}_{n+1}$.
    \STATE Apply the Metropolis-Hastings accept-reject decision.
    \STATE Set $M\gets H(q_n, p_n) - H(\tilde{q}_{n+1}, \tilde{p}_{n+1})$ and sample $u\sim\mathrm{Uniform}(0, 1)$.
    \IF{$u < M$}
    \STATE Accept the proposal and set $(q_{n+1}, p_{n+1}) \gets (\tilde{q}_{n+1}, \tilde{p}_{n+1})$.
    \ELSE
    \STATE Reject the proposal and set $(q_{n+1}, p_{n+1}) \gets (q_n, p_n)$.
    \ENDIF
    \STATE {\bf Return:} The next state of the Markov chain $(q_{n+1}, p_{n+1})$.
  \end{algorithmic}
\end{algorithm}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/algorithms/leapfrog.tex <==
\begin{algorithm}[t!]
  \caption{The leapfrog integrator, which is a volume-preserving, reversible,
    second-order accurate numerical integrator for separable Hamiltonians. The
    leapfrog integrator is fully explicit, involving no fixed point iterations,
    giving it an important computational advantage over Riemannian methods.}
  \label{alg:leapfrog}
  \begin{algorithmic}
    \STATE {\bf Input:} An initial state $(q_n, p_n)\in \R^m\times\R^m$, a smooth, separable Hamiltonian $H:\R^m\times\R^m\to\R$, a step-size $\epsilon\in\R$.
    \STATE Compute an explicit half-step in the momentum variable,
    \begin{align}
      p_{n+1/2} = p_n - \frac{\epsilon}{2} \nabla_q H(q_n, p_{n}).
    \end{align}
    \STATE Compute an explicit full step in the position variable,
    \begin{align}
      q_{n+1} = q_n + \epsilon\nabla_p H(q_n, p_{n+1/2}).
    \end{align}
    \STATE Apply an explicit half-step in the momentum variable,
    \begin{align}
      p_{n+1} = p_{n+1/2} - \frac{\epsilon}{2} \nabla_q H(q_{n+1}, p_{n+1/2}).
    \end{align}
    \STATE {\bf Return:} $(q_{n+1}, p_{n+1})$, the next position in phase-space along the integrated trajectory.
  \end{algorithmic}
\end{algorithm}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/algorithms/moral-implicit-midpoint.tex <==
\begin{algorithm}[t!]
  \caption{The implicit midpoint integrator for producing a symmetric,
    volume-preserving, second-order accurate to Hamilton's equations of motion
    for an arbitrary smooth Hamiltonian. This procedure implements a single step
    of the implicit midpoint integrator, which may then be repeatedly
    composed in order to integrate over longer trajectories.}
  \label{alg:moral-implicit-midpoint}
  \begin{algorithmic}
    \STATE {\bf Input:} An initial state $(q_n, p_n)\in \R^m\times\R^m$, a smooth Hamiltonian $H:\R^m\times\R^m\to\R$, a step-size $\epsilon\in\R$.
    \STATE Solve the implicit equation,
    \begin{align}
      \label{eq:moral-implicit-midpoint} \begin{pmatrix} q_{n+1} \\ p_{n+1} \end{pmatrix} &= \begin{pmatrix} q_n \\ p_n \end{pmatrix} + \epsilon \begin{pmatrix} \nabla_p H(\bar{q}_n, \bar{p}_n) \\ -\nabla_q H(\bar{q}_n, \bar{p}_n) \end{pmatrix} \\
      \bar{q}_n &= \frac{q_{n+1} + q_n}{2} \\
      \bar{p}_n &= \frac{p_{n+1} + p_n}{2}
    \end{align}
    \STATE {\bf Return:} $(q_{n+1}, p_{n+1})$, the next position in phase-space along the integrated trajectory.
  \end{algorithmic}
\end{algorithm}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/algorithms/moral-leapfrog.tex <==
\begin{algorithm}[t!]
  \caption{The generalized leapfrog integrator for producing a symmetric,
    volume-preserving, second-order accurate to Hamilton's equations of motion
    for an arbitrary smooth Hamiltonian. This procedure implements a single step
    of the generalized leapfrog integrator, which may then be repeatedly
    composed in order to integrate over longer trajectories.}
  \label{alg:moral-leapfrog}
  \begin{algorithmic}
    \STATE {\bf Input:} An initial state $(q_n, p_n)\in \R^m\times\R^m$, a smooth Hamiltonian $H:\R^m\times\R^m\to\R$, a step-size $\epsilon\in\R$.
    \STATE Compute a half-step in the momentum variable,
    \begin{align}
      \label{eq:moral-leapfrog-momentum-implicit} p_{n+1/2} = p_n - \frac{\epsilon}{2} \nabla_q H(q_n, p_{n+1/2}).
    \end{align}
    \STATE Compute a full step in the position variable,
    \begin{align}
      \label{eq:moral-leapfrog-position} q_{n+1} = q_n + \frac{\epsilon}{2} \paren{\nabla_p H(q_n, p_{n+1/2}) + \nabla_p H(q_{n+1}, p_{n+1/2})}.
    \end{align}
    \STATE Apply an explicit half-step update to the momentum variable,
    \begin{align}
      \label{eq:moral-leapfrog-momentum-explicit} p_{n+1} = p_{n+1/2} - \frac{\epsilon}{2} \nabla_q H(q_{n+1}, p_{n+1/2}).
    \end{align}
    \STATE {\bf Return:} $(q_{n+1}, p_{n+1})$, the next position in phase-space along the integrated trajectory.
  \end{algorithmic}
\end{algorithm}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/algorithms/threshold-leapfrog.tex <==
\begin{algorithm}[t!]
  \caption{In practice the generalized leapfrog integrator is implemented with
    fixed point iterations, as advocated by \citet{}, to resolve the
    implicitly-defined relations. As a result, the integrator violates
    reversibility and volume preservation above the level of numerical
    precision.}
  \label{alg:threshold-leapfrog}
  \begin{algorithmic}
    \STATE {\bf Input:} An initial state $(q_n, p_n)\in \R^m\times\R^m$, a
    smooth Hamiltonian $H:\R^m\times\R^m\to\R$, a step-size $\epsilon\in\R$, a
    convergence threshold $\delta > 0$, a maximal number of allowable fixed
    point iterations $M\in \mathbb{N}$.
    \STATE Compute a half-step in the momentum variable:
    \STATE Set $p_{n+1/2} \gets p_n$, $l_p \gets 0$, $\Delta_p \gets \infty$.
    \WHILE{$\Delta_p > \delta$ and $l_p < M$}
    \STATE
    \begin{align}
      \label{eq:generalized-leapfrog-momentum-fixed-point-i} p_{n+1/2}' &\gets p_n - \frac{\epsilon}{2} \nabla_q H(q_n, p_{n+1/2}) \\
      \label{eq:generalized-leapfrog-momentum-fixed-point-ii} \Delta_p &\gets \Vert p_{n+1/2}' - p_{n+1/2}\Vert_\infty
    \end{align}
    \STATE Assign $p_{n+1/2} \gets p_{n+1/2}'$ and set $l_p \gets l_p + 1$.
    \ENDWHILE
    \STATE Compute a full step in the position variable:
    \STATE Set $q_{n+1} \gets q_n$, $l_q\gets 0$, $\Delta_q \gets \infty$.
    \WHILE{$\Delta_q > \delta$ and $l_q < M$}
    \STATE
    \begin{align}
      \label{eq:generalized-leapfrog-position-fixed-point-i} q_{n+1}' &\gets q_n + \frac{\epsilon}{2} \paren{\nabla_p H(q_n, p_{n+1/2}) + \nabla_p H(q_{n+1}, p_{n+1/2})} \\
      \label{eq:generalized-leapfrog-position-fixed-point-ii} \Delta_q &\gets \Vert q_{n+1}' - q_{n+1}\Vert_\infty
    \end{align}
    \STATE Assign $q_{n+1} \gets q_{n+1}'$ and set $l_q \gets l_q + 1$.
    \ENDWHILE
    \STATE Compute an explicit half-step update to the momentum variable:
    \begin{align}
      p_{n+1} \gets p_{n+1/2} - \frac{\epsilon}{2} \nabla_q H(q_{n+1}, p_{n + 1/2}).
    \end{align}
    \STATE {\bf Return:} $(q_{n+1}, p_{n+1})$, the next position in phase-space along the integrated trajectory.
  \end{algorithmic}
\end{algorithm}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/banana/computational-effort-ergodicity.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/banana/num-fixed-point-position.pdf}
    \caption{Number of fixed point iterations for position variable.}
    \label{subfig:banana-fixed-point-position}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/banana/num-fixed-point-momentum.pdf}
    \caption{Number of fixed point iterations for momentum variable.}
    \label{subfig:banana-fixed-point-momentum}
  \end{subfigure}
  
  \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{images/banana/kolmogorov-smirnov.pdf}
    \caption{Ergodicity of RMHMC and HMC}
    \label{subfig:banana-ergodicity}
  \end{subfigure}
  
  \caption{Visualization of the computational effort required to sample with RMHMC from the banana posterior. We show the number of fixed point iterations required to compute the two implicit steps of the generalized leapfrog integrator as well as the distribution of Kolmogorov-Smirnov statistics over variable thresholds. The maximum Kolmogorov-Smirnov statistic of Euclidean HMC with a step-size of $0.1$ is shown as a dashed blue line.}
\end{figure}

==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/banana/dual-averaging.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/dual-averaging-loss.pdf}
    \caption{$L_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/dual-averaging-threshold.pdf}
    \caption{$\delta_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/dual-averaging-function.pdf}
    \caption{Monte Carlo $B(\delta)$}
    \label{subfig:banana-dual-averaging-function}
  \end{subfigure}
  \caption{The use of Ruppert averaging in the banana-shaped distribution to adaptively set the convergence threshold to achieve eight decimal digits of similarity compared to a transition kernel with a threshold of $1\times 10^{-10}$. We show a Monte Carlo approximation to $B(\delta)$, which appears smooth, monotonically increasing. The value of $\delta$ satisfying $B(\delta)=0$ is approximately $\delta = 1\times 10^{-8}$, which is approximately the value of produced by Ruppert averaging.}
  \label{fig:banana-dual-averaging}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/banana/extra-ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/biau.pdf}
    \caption{Biau Metric}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/mmd.pdf}
    \caption{$\mathrm{MMD}_u^2$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/sw.pdf}
    \caption{Sliced Wasserstein}
  \end{subfigure}
  \caption{Additional measures of ergodicity in the banana-shaped distribution. For thresholds smaller than $1\times10^{-2}$, the Riemannian methods produce a modest improvement in the ergodicity of the samples produced by the Markov chain. In computing the MMD metric, we employ a bandwidth of 1.727.}
  \label{fig:banana-extra-ergodicity}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/banana/metrics.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/banana/absolute-reversibility.pdf}
    \caption{Error in Reversibility}
    \label{subfig:banana-reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/banana/jacobian-determinant.pdf}
    \caption{Error in Volume-Preservation}
    \label{subfig:banana-jacobian-determinant}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/banana/transition-kernel-distance-.pdf}
    \caption{Difference in Transition Kernel}
    \label{subfig:banana-transition-difference}
  \end{subfigure}
  \caption{Visualization of the error in reversibility (see
    \cref{subfig:banana-reversibility}), error in
    volume-preservation (see
    \cref{subfig:banana-jacobian-determinant}), and the number of
    decimal digits of similarity in transition kernels (see
    \cref{subfig:banana-transition-difference}) for variable
    thresholds in the banana posterior distribution.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/banana/trajectory.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/banana/threshold-precondition.pdf}
    \caption{Generalized Leapfrog Trajectories}
    \label{subfig:banana-trajectory-threshold-precondition}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/banana/position-deviation.pdf}
    \caption{Error in the Position Variable}
    \label{subfig:banana-trajectory-position-deviation}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/banana/energy-deviation.pdf}
    \caption{Conservation of Hamiltonian Energy}
    \label{subfig:banana-trajectory-energy-deviation}
  \end{subfigure}
  \caption{In \cref{subfig:banana-trajectory-threshold-precondition} we
    visualize the trajectories produced by the generalized leapfrog integrator
    with variable thresholds. A trajectory of the leapfrog integrator using a
    separable Hamiltonian is shown for comparison, which also reveals the
    preconditioning effect. Although the trajectories in \cref{subfig:banana-trajectory-threshold-precondition} are qualitatively similar, in
    \cref{subfig:banana-trajectory-position-deviation} we measure the
    number of decimal digits conserved in the position variable for differing
    thresholds relative to the generalized leapfrog integrator with threshold
    $1\times 10^{-10}$; this reveals the extent to which the trajectories are differentiated by the choice of threshold. The approximate conservation of the Hamiltonian is
    violated is visualized in \cref{subfig:banana-trajectory-energy-deviation}.}
  \label{fig:banana-trajectory}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/cox-poisson/computational-effort.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/num-fixed-point-position.pdf}
    \caption{Position fixed point iterations}
    \label{subfig:cox-poisson-fixed-point-position}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/num-fixed-point-momentum.pdf}
    \caption{Momentum fixed point iterations}
    \label{subfig:cox-poisson-fixed-point-momentum}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/transition-kernel-distance-.pdf}
    \caption{Difference in Transition Kernel}
    \label{subfig:cox-poisson-transition-difference}
  \end{subfigure}
  \caption{Visualization of the number of fixed point iterations required to compute the implicit updates to position and momentum required by the generalized leapfrog integrator in the log-Gaussian Cox-Poisson model. The number of decimal digits of similarity in transition kernels are shown in  \cref{subfig:cox-poisson-transition-difference} for variable thresholds.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/cox-poisson/cox-poisson.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=\textwidth]{images/cox-poisson/cox-poisson.png}
  \caption{Visualization of the posterior mean (in the first row) and posterior standard deviation (in the second row) of the spatial latent process wherein the kernel parameters $(\sigma^2,\beta)$ are sampled by RMHMC with variable thresholds. Within the Riemannian algorithms with varying thresholds, these quantities are visually indistinguishable. However, one does observe differences in the posterior standard deviation when comparing RMHMC to Euclidean HMC.}
  \label{fig:cox-poisson-cox-poisson}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/cox-poisson/metrics.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/absolute-reversibility.pdf}
    \caption{Error in Reversibility}
    \label{subfig:cox-poisson-reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/jacobian-determinant.pdf}
    \caption{Error in Volume-Preservation}
    \label{subfig:cox-poisson-jacobian-determinant}
  \end{subfigure}
  
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/hyper-parameter-minimum-ess-per-second-1.pdf}
    \caption{$\beta$}
    \label{subfig:cox-poisson-beta-ess-per-second}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/hyper-parameter-minimum-ess-per-second-2.pdf}
    \caption{$\sigma$}
    \label{subfig:cox-poisson-sigma-ess-per-second}
  \end{subfigure}

  \caption{Visualization of the error in reversibility (see
    \cref{subfig:cox-poisson-reversibility}) and error in
    volume-preservation (see
    \cref{subfig:cox-poisson-jacobian-determinant}) in the log-Gaussian Cox-Poisson posterior. We also illustrate the ESS per second for sampling the hyperparameters of the Cox-Poisson model and a comparison against a Euclidean HMC method.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fitzhugh-nagumo/computational-effort.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/num-fixed-point-position.pdf}
    \caption{Number of fixed point iterations for position variable.}
    \label{subfig:fitzhugh-nagumo-fixed-point-position}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/num-fixed-point-momentum.pdf}
    \caption{Number of fixed point iterations for momentum variable.}
    \label{subfig:fitzhugh-nagumo-fixed-point-momentum}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/transition-kernel-distance-.pdf}
    \caption{Difference in Transition Kernel}
    \label{subfig:fitzhugh-nagumo-transition-difference}
  \end{subfigure}
  \caption{Visualization of the error in reversibility (see
    \cref{subfig:fitzhugh-nagumo-reversibility}), error in
    volume-preservation (see
    \cref{subfig:fitzhugh-nagumo-jacobian-determinant}), and the number of
    decimal digits of similarity in transition kernels (see
    \cref{subfig:fitzhugh-nagumo-transition-difference}) for variable
    thresholds in the Fitzhugh-Nagumo posterior distribution.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fitzhugh-nagumo/dual-averaging.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/dual-averaging-loss.pdf}
    \caption{$L_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/dual-averaging-threshold.pdf}
    \caption{$\delta_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/dual-averaging-function.pdf}
    \caption{Monte Carlo $B(\delta)$}
  \end{subfigure}
  \caption{The use of Ruppert averaging in the Fitzhugh-Nagumo posterior distribution to adaptively set the convergence threshold to achieve four decimal digits of similarity compared to a transition kernel with a threshold of $1\times 10^{-10}$.  We show a Monte Carlo approximation to $B(\delta)$, which appears smooth, monotonically increasing. The value of $\delta$ satisfying $B(\delta)=0$ is approximately $\delta = 1\times 10^{-5.3}$, which is approximately the value of produced by Ruppert averaging.}
  \label{fig:fitzhugh-nagumo-dual-averaging}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fitzhugh-nagumo/extra-ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/mmd.pdf}
    \caption{$\mathrm{MMD}_u^2$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/sw.pdf}
    \caption{Sliced Wasserstein}
  \end{subfigure}
  \caption{Additional measures of ergodicity in the Fitzhugh-Nagumo differential equation model. In this example, the $\mathrm{MMD}_u^2$ statistic indicates that a threshold of $1\times 10^{-2}$ has the smallest value of the squared maximum mean discrepancy. This is in contrast to the Kolmogorov-Smirnov and sliced Wasserstein metrics, which indicate the ergodicity improves to a threshold of $1\times 10^{-3}$. In the MMD statistic we use a kernel bandwidth of 0.088.}
  \label{fig:fitzhugh-nagumo-extra-ergodicity}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fitzhugh-nagumo/fitzhugh-nagumo.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/fitzhugh-nagumo.png}
  \caption{Visualization of the posterior mean of $v_t$ (in blue) and $r_t$ (in orange) in the Fitzhugh-Nagumo posterior distribution. The posterior means are visually indistinguishable irrespective of the convergence tolerance used in RMHMC.}
  \label{fig:fitzhugh-nagumo-fitzhugh-nagumo}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fitzhugh-nagumo/incorrect-metrics.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/incorrect/absolute-reversibility.pdf}
    \caption{Error in Reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/incorrect/jacobian-determinant.pdf}
    \caption{Error in Volume-Preservation}
  \end{subfigure}
  
  \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/incorrect/kolmogorov-smirnov.pdf}
    \caption{Ergodicity of RMHMC with incorrectly specified partial derivatives}
    \label{subfig:fitzhugh-nagumo-incorrect-ergodicity}
  \end{subfigure}
  \caption{Visualization of how a failure to respect the symmetry of partial derivatives yields severely degraded sample quality; indeed, the target distribution may be warped. Although reversibility can be reduced by a decreasing threshold, the property of volume-preservation cannot be recovered irrespective of threshold. As a consequence, the RMHMC algorithm is no longer ergodic for the target distribution, which is reflected in the degraded ergodicity measure.}
  \label{fig:fitzhugh-nagumo-incorrect-metrics}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fitzhugh-nagumo/metrics-ergodicity.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/absolute-reversibility.pdf}
    \caption{Error in Reversibility}
    \label{subfig:fitzhugh-nagumo-reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/jacobian-determinant.pdf}
    \caption{Error in Volume-Preservation}
    \label{subfig:fitzhugh-nagumo-jacobian-determinant}
  \end{subfigure}
  
  \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/kolmogorov-smirnov.pdf}
    \caption{Ergodicity of RMHMC and HMC}
    \label{subfig:fitzhugh-nagumo-ergodicity}
  \end{subfigure}
  \caption{Visualization of the computational effort required to sample with RMHMC from the Fitzhugh-Nagumo posterior. We show the number of fixed point iterations required to compute the two implicit steps of the generalized leapfrog integrator as well as the distribution of Kolmogorov-Smirnov statistics over variable thresholds.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fixed-point-vs-newton/ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/kolmogorov-smirnov-vs-newton.pdf}
    \caption{Banana}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/kolmogorov-smirnov-vs-newton.pdf}
    \caption{Fitzhugh-Nagumo}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/kolmogorov-smirnov-vs-newton.pdf}
    \caption{Student-$t$}
  \end{subfigure}

  \caption{We visualize the ergodicity properties for the three implementations of RMHMC. In the casae where Newton's method is employed for resolving the implicit updates to momentum and position, the ergodicity of the method is essentially constant with respect to the convergence tolerance. However, this is not desirable in the case of the banana-shaped posterior distribution, wherein ergodicity failures result from severe violations of reversibility and volume preservation in some cases.}
  \label{fig:fixed-point-vs-newton-ergodicity}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fixed-point-vs-newton/ess-same.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/hyper-parameter-minimum-ess-per-second-vs-newton-1.pdf}
    \caption{(SV) $\phi$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/hyper-parameter-minimum-ess-per-second-vs-newton-2.pdf}
    \caption{(SV) $\beta$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/hyper-parameter-minimum-ess-per-second-vs-newton-3.pdf}
    \caption{(SV) $\sigma^2$}
  \end{subfigure}
  
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/hyper-parameter-minimum-ess-per-second-vs-newton-1.pdf}
    \caption{(CP) $\beta$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/cox-poisson/hyper-parameter-minimum-ess-per-second-vs-newton-2.pdf}
    \caption{(CP) $\sigma$}
  \end{subfigure}
  
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/minimum-ess-per-second-vs-newton-1.pdf}
    \caption{(FN) $a$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/minimum-ess-per-second-vs-newton-2.pdf}
    \caption{(FN) $b$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/minimum-ess-per-second-vs-newton-3.pdf}
    \caption{(FN) $c$}
  \end{subfigure}  
  
  \caption{Three circumstances in which Newton's method produced performance comparable to fixed point iteration when resolving the implicit update to the momentum. In these cases, Newton's method may actually be the preferred method, since it is somewhat less sensitive to the convergence tolerance. In the first row we show results for the stochastic volatility model (SV); the second row shows the log-Gauss Cox-Poisson model (CP); the third row shows results for the Fitzhugh-Nagumo differential equation model (FN).}
  \label{fig:fixed-point-vs-newton-ess-same}
\end{figure}

==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fixed-point-vs-newton/ess-worse.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{images/banana/minimum-ess-per-second-vs-newton.pdf}
    \caption{Banana}
    \label{subfig:fixed-point-vs-newton-ess-wose-banana}
  \end{subfigure}

  \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{images/logistic-regression/minimum-ess-per-second-vs-newton.pdf}
    \caption{Logistic Regression}
  \end{subfigure}

  \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{images/t/minimum-ess-per-second-vs-newton.pdf}
    \caption{Student-$t$}
  \end{subfigure}
  
  \caption{Three circumstances are shown wherein the use of Newton's method to resolve the implicit update to the momentum resulted in degraded sampling efficiency due to the higher computational burden of Newton's method compared to fixed point iteration. In the banana-shaped distribution, although the posterior is only two-dimensional, significant computation is wasted while searching for solutions to the momentum update that do not exist.}
  \label{fig:fixed-point-vs-newton-ess-worse}
\end{figure}

==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fixed-point-vs-newton/jacobian-determinant.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/jacobian-determinant-vs-newton.pdf}
    \caption{Banana}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic-regression/jacobian-determinant-vs-newton.pdf}
    \caption{Logistic Regression}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/jacobian-determinant-vs-newton.pdf}
    \caption{Stochastic Volatility}
  \end{subfigure}
  
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/jacobian-determinant-vs-newton.pdf}
    \caption{Cox-Poisson}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/jacobian-determinant-vs-newton.pdf}
    \caption{Fitzhugh-Nagumo}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/jacobian-determinant-vs-newton.pdf}
    \caption{Student-$t$}
  \end{subfigure}

  \caption{We illustrate the dependency of the Jacobian determinant metric on the procedure used to resolve the implicit updates to momentum and position. Employing Newton's method to update both the position and the momentum variables in the generalized leapfrog integrator yields faster convergence toward a volume-preserving proposal.}
  \label{fig:fixed-point-vs-newton-jacobian-determinant}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fixed-point-vs-newton/momentum-iterations.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/num-fixed-point-momentum-vs-newton.pdf}
    \caption{Banana}
    \label{subfig:fixed-point-vs-newton-banana}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic-regression/num-fixed-point-momentum-vs-newton.pdf}
    \caption{Logistic Regression}
    \label{subfig:fixed-point-vs-newton-logistic}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/num-fixed-point-momentum-vs-newton.pdf}
    \caption{Stochastic Volatility}
    \label{subfig:fixed-point-vs-newton-stochastic-volatility}
  \end{subfigure}
  
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/num-fixed-point-momentum-vs-newton.pdf}
    \caption{Cox-Poisson}
    \label{subfig:fixed-point-vs-newton-cox-poisson}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/num-fixed-point-momentum-vs-newton.pdf}
    \caption{Fitzhugh-Nagumo}
    \label{subfig:fixed-point-vs-newton-fitzhugh-nagumo}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/num-fixed-point-momentum-vs-newton.pdf}
    \caption{Student-$t$}
    \label{subfig:fixed-point-vs-newton-student-t}
  \end{subfigure}

  \caption{We compute the number of iterations required to resolve the implicit updates to the momentum variable when using either fixed point iteration or Newton's method. We report the mean number of iterations with error bars showing dispersion about the mean. In each circumstance, Newton's method converges faster than fixed point iterations, reflecting its superior order of convergence. Only around three iterations of Newton's method are required on average in each example. We observe that in many cases, Newton's method appears to be less sensitive to the convergence tolerance.}
  \label{fig:fixed-point-vs-newton-iterations}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/fixed-point-vs-newton/reversibility.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/absolute-reversibility-vs-newton.pdf}
    \caption{Banana}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic-regression/absolute-reversibility-vs-newton.pdf}
    \caption{Logistic Regression}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/absolute-reversibility-vs-newton.pdf}
    \caption{Stochastic Volatility}
  \end{subfigure}
  
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/absolute-reversibility-vs-newton.pdf}
    \caption{Cox-Poisson}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/absolute-reversibility-vs-newton.pdf}
    \caption{Fitzhugh-Nagumo}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/absolute-reversibility-vs-newton.pdf}
    \caption{Student-$t$}
  \end{subfigure}

  \caption{We illustrate the dependency of the reversibility metric on the procedure used to resolve the implicit updates to momentum and position. In most examples, employing Newton's method to update both the position and the momentum variables in the generalized leapfrog integrator produced faster convergence to, and better respect for, reversibility of the proposal up to numerical precision.}
  \label{fig:fixed-point-vs-newton-reversibility}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/jacobian-determinant-perturbation.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/perturbation.pdf}
    \caption{Banana}
    \label{subfig:jacobian-determinant-banana}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic-regression/perturbation.pdf}
    \caption{Logistic Regression}
    \label{subfig:jacobian-determinant-logistic}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/perturbation.pdf}
    \caption{Neal Funnel}
    \label{subfig:jacobian-determinant-neal-funnel}
  \end{subfigure}

  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/perturbation.pdf}
    \caption{Stochastic Volatility}
    \label{subfig:jacobian-determinant-stochastic-volatility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/perturbation.pdf}
    \caption{Cox-Poisson}
    \label{subfig:jacobian-determinant-cox-poisson}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/perturbation.pdf}
    \caption{Fitzhugh-Nagumo}
    \label{subfig:jacobian-determinant-fitzhugh-nagumo}
  \end{subfigure}

  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/perturbation.pdf}
    \caption{Student-$t$}
    \label{subfig:jacobian-determinant-student-t}
  \end{subfigure}

  \caption{We show how the estimated volume preservation of the generalized leapfrog integrator is affected by the choice of finite difference perturbation size. We report the degree of volume-preservation for the generalized leapfrog integrator with a convergence threshold of $\delta= 1\times 10^{-9}$.}
  \label{fig:jacobian-determinant-perturbation}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/logistic-regression/metrics.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/logistic-regression/absolute-reversibility.pdf}
    \caption{Error in Reversibility}
    \label{subfig:logistic-regression-reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/logistic-regression/jacobian-determinant.pdf}
    \caption{Error in Volume-Preservation}
    \label{subfig:logistic-regression-jacobian-determinant}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/logistic-regression/transition-kernel-distance-.pdf}
    \caption{Difference in Transition Kernel}
    \label{subfig:logistic-regression-transition-difference}
  \end{subfigure}
  \caption{Visualization of the error in reversibility (see \cref{subfig:logistic-regression-reversibility}), error in volume-preservation (see \cref{subfig:logistic-regression-jacobian-determinant}), and the number of decimal digits of similarity in transition kernels (see \cref{subfig:logistic-regression-transition-difference}) for variable thresholds in the logistic posterior distribution.}
  \label{fig:logistic-regression-metrics}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/neal-funnel/computational-effort.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/neal-funnel/num-fixed-point-position.pdf}
    \caption{Number of fixed point iterations for position variable.}
    \label{subfig:neal-funnel-fixed-point-position}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/neal-funnel/num-fixed-point-momentum.pdf}
    \caption{Number of fixed point iterations for momentum variable.}
    \label{subfig:neal-funnel-fixed-point-momentum}
  \end{subfigure}
  \caption{Visualization of the computational effort required to sample with RMHMC from Neal's funnel distribution. We show the number of fixed point iterations required to compute the two implicit steps of the generalized leapfrog integrato.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/neal-funnel/dual-averaging.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/dual-averaging-loss.pdf}
    \caption{$L_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/dual-averaging-threshold.pdf}
    \caption{$\delta_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/dual-averaging-function.pdf}
    \caption{Monte Carlo $B(\delta)$}
  \end{subfigure}
  \caption{The use of Ruppert averaging in Neal's funnel distribution to adaptively set the convergence threshold to achieve six decimal digits of similarity compared to a transition kernel with a threshold of $1\times 10^{-10}$. We show a Monte Carlo approximation to $B(\delta)$, which appears smooth, monotonically increasing. The value of $\delta$ satisfying $B(\delta)=0$ is approximately $\delta = 1\times 10^{-6.5}$, which is somewhat greater than the value of $1\times 10^{-7}$ produced by Ruppert averaging.}
  \label{fig:neal-funnel-dual-averaging}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/neal-funnel/extra-ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/mmd.pdf}
    \caption{$\mathrm{MMD}_u^2$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/sw.pdf}
    \caption{Sliced Wasserstein}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/convergence.pdf}
    \caption{Ergodic Convergence}
  \end{subfigure}
  \caption{Additional measures of ergodicity in Neal's funnel distribution. According to the Kolmogorov-Smirnov and $\mathrm{MMD}_u^2$ statistics, the Riemannian methods with a threshold of $1\times10^{-1}$ are competitive with the best-performing Euclidean methods. However, by the sliced Wasserstein metric, all Riemannian methods have better ergodicity compared to the Euclidean variants. In any event, all metrics agree that ergodicity performance is essentially constant for thresholds less than $1\times 10^{-2}$. We show convergence of independent Markov chains in the marginal distribution of $v$ which is $\mathrm{Normal}(0, 3^2)$. We see that convergence of Riemannian methods is faster than for HMC; however, when employing the largest threshold, one can observe the bias in the stationary distribution. In computing the MMD statistic, we use a kernel bandwidth of 8.4.}
  \label{fig:neal-funnel-extra-ergodicity}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/neal-funnel/metrics.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/neal-funnel/absolute-reversibility.pdf}
    \caption{Error in Reversibility}
    \label{subfig:neal-funnel-reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/neal-funnel/jacobian-determinant.pdf}
    \caption{Error in Volume-Preservation}
    \label{subfig:neal-funnel-jacobian-determinant}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/neal-funnel/transition-kernel-distance-alpha-10000.0.pdf}
    \caption{Difference in Transition Kernel}
    \label{subfig:neal-funnel-transition-difference}
  \end{subfigure}
  \caption{Visualization of the error in reversibility (see \cref{subfig:neal-funnel-reversibility}), error in volume-preservation (see \cref{subfig:neal-funnel-jacobian-determinant}), and the number of decimal digits of similarity in transition kernels (see \cref{subfig:neal-funnel-transition-difference}) for variable thresholds in Neal's funnel distribution with $10 + 1$ dimensions.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/reversibility-relative-error.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/banana/relative-reversibility.pdf}
    \caption{Banana}
    \label{subfig:relative-error-banana}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/logistic-regression/relative-reversibility.pdf}
    \caption{Logistic Regression}
    \label{subfig:relative-error-logistic}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/neal-funnel/relative-reversibility.pdf}
    \caption{Neal Funnel}
    \label{subfig:relative-error-neal-funnel}
  \end{subfigure}

  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility/relative-reversibility.pdf}
    \caption{Stochastic Volatility}
    \label{subfig:relative-error-stochastic-volatility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/cox-poisson/relative-reversibility.pdf}
    \caption{Cox-Poisson}
    \label{subfig:relative-error-cox-poisson}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/correct/relative-reversibility.pdf}
    \caption{Fitzhugh-Nagumo}
    \label{subfig:relative-error-fitzhugh-nagumo}
  \end{subfigure}

  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/relative-reversibility.pdf}
    \caption{Student-$t$}
    \label{subfig:relative-error-student-t}
  \end{subfigure}

  \caption{We measure the relative error in reversibility by normalizing the absolute reversibility error by the norm of initial condition. This measure contextualizes the reversibility error in terms of the scale of the distribution.}
  \label{fig:reversibility-relative-error}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/stochastic-volatility/computational-effort.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/num-fixed-point-position.pdf}
    \caption{Position fixed point iterations}
    \label{subfig:stochastic-volatility-fixed-point-position}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/num-fixed-point-momentum.pdf}
    \caption{Momentum fixed point iterations}
    \label{subfig:stochastic-volatility-fixed-point-momentum}
  \end{subfigure}

  \caption{Visualization of the number of fixed point iterations required to compute the implicit updates to position and momentum required by the generalized leapfrog integrator in the stochastic volatility model.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/stochastic-volatility/ess-per-second.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/hyper-parameter-minimum-ess-per-second-1.pdf}
    \caption{$\phi$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/hyper-parameter-minimum-ess-per-second-2.pdf}
    \caption{$\beta$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/hyper-parameter-minimum-ess-per-second-3.pdf}
    \caption{$\sigma^2$}
  \end{subfigure}
  \caption{Visualization of the ESS per second for the three latent parameters of the stochastic volatility model.}
  \label{fig:stochastic-volatility-ess-per-second}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/stochastic-volatility/metrics.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/absolute-reversibility.pdf}
    \caption{$\log_{10}$ reversibility error}
    \label{subfig:stochastic-volatility-reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/jacobian-determinant.pdf}
    \caption{$\log_{10}$ volume-preservation error}
    \label{subfig:stochastic-volatility-jacobian-determinant}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/stochastic-volatility/transition-kernel-distance-.pdf}
    \caption{$\log_{10}$ transition kernel difference}
    \label{subfig:stochastic-volatility-transition-difference}
  \end{subfigure}
  \caption{Visualization of the error in reversibility (see \cref{subfig:stochastic-volatility-reversibility}), error in volume-preservation (see \cref{subfig:stochastic-volatility-jacobian-determinant}), and the number of decimal digits of similarity in transition kernels (see \cref{subfig:stochastic-volatility-transition-difference}) for variable thresholds in the stochastic volatility posterior.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/stochastic-volatility/stochastic-volatility.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=\textwidth]{images/stochastic-volatility/stochastic-volatility.png}
  \caption{Visualization of the posterior distribution over the stochastic
    volatilities wherein the process hyperparameters $(\sigma^2,\phi,\beta)$ are
    sampled by RMHMC with variable threshold. Visually, the posterior
    distributions are indistinguishable.}
  \label{fig:stochastic-volatility-stochastic-volatility}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/t/dual-averaging.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/dual-averaging-loss.pdf}
    \caption{$L_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/dual-averaging-threshold.pdf}
    \caption{$\delta_n$ Sequence}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/dual-averaging-function.pdf}
    \caption{Monte Carlo $B(\delta)$}
  \end{subfigure}
  \caption{The use of Ruppert averaging in the multiscale Student-$t$ distribution to adaptively set the convergence threshold to achieve eight decimal digits of similarity compared to a transition kernel with a threshold of $1\times 10^{-10}$. We show a Monte Carlo approximation to $B(\delta)$, which appears smooth, monotonically increasing. The value of $\delta$ satisfying $B(\delta)=0$ is approximately $\delta = 1\times 10^{-7.83}$, which is somewhat greater than the value of $1\times 10^{-8}$ produced by Ruppert averaging. We note that the function $B(\delta)$ is approximately constant over the interval $[-3, -2]$; this could present difficulty in optimizing thresholds in this range since it violates the fourth assumption for convergence of the Robbins-Monro algorithm.}
  \label{fig:student-t-dual-averaging}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/t/extra-ergodicity.tex <==
\begin{figure}[t!]
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/mmd.pdf}
    \caption{$\mathrm{MMD}_u^2$}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/sw.pdf}
    \caption{Sliced Wasserstein}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/t/convergence.pdf}
    \caption{Ergodic Convergence}
  \end{subfigure}
  \caption{Additional measures of ergodicity in the multivariate Student-$t$ distribution. In the presence of the multiscale phenomena, the Euclidean HMC algorithms cannot achieve the same level of ergodicity as the Riemannian algorithms except in the case wherein a very large convergence tolerance is used in RMHMC. When $\sigma^2=1\times 10^4$, we also show convergence of the dimension with largest variation, whose marginal is $t(5, \sigma^2)$. The Riemannian methods exhibit faster convergence compared to HMC. For $\sigma^2=1\times 10^4$, the MMD statistic uses a bandwidth of 110.72 in the squared exponential kernel.}
  \label{fig:t-extra-ergodicity}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/t/metrics.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/t/absolute-reversibility.pdf}
    \caption{Error in Reversibility}
    \label{subfig:t-reversibility}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/t/jacobian-determinant.pdf}
    \caption{Error in Volume-Preservation}
    \label{subfig:t-jacobian-determinant}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/t/transition-kernel-distance-.pdf}
    \caption{Difference in Transition Kernel}
    \label{subfig:t-transition-difference}
  \end{subfigure}
  \caption{Visualization of the error in reversibility (see \cref{subfig:t-reversibility}), error in volume-preservation (see \cref{subfig:t-jacobian-determinant}), and the number of decimal digits of similarity in transition kernels (see \cref{subfig:t-transition-difference}) for variable thresholds in a multivariate Student-$t$ distribution with $\sigma^2 = 10,000$.}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/figures/t/multiscale-phenomena.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/t/kolmogorov-smirnov-scale.pdf}
    \caption{Error in Reversibility}
    \label{subfig:t-kolmogorov-smirnov-scale}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/t/effective-sample-size-per-second-scale.pdf}
    \caption{Error in Volume-Preservation}
    \label{subfig:t-ess-per-second-scale}
  \end{subfigure}

  \caption{Visualization of how multiscale properties of a target multivariate Student-$t$ distribution affect the ergodicity and computational efficiency of the Euclidean HMC and RMHMC algorithms. In the prescence of severe multiscale attributes of the posterior, Euclidean methods of HMC exhibit poor sampling performance by these metrics.}
  \label{fig:t-multiscale-phenomena}
\end{figure}


==> On Numerical Considerations for Riemannian Manifold Hamiltonian Monte Carlo/tables/posteriors.tex <==
\begin{table}[t]
\begin{tabular}{@{}l|lllll@{}}
\toprule
Posterior                                                           & \# Dimensions & \# Samples & Metric                            & Hierarchical          & \begin{tabular}[c]{@{}l@{}}Exact\\ Gradients\end{tabular} \\ \midrule
Banana                                                              & 2             & 1,000,000  & Fisher Information + Hessian      & \xmark & \cmark                                     \\
\begin{tabular}[c]{@{}l@{}}Logistic\\ Regression\end{tabular}       & 14 + 1        & 100,000    & Fisher Information + Hessian      & \cmark & \cmark                                     \\
Neal's Funnel                                                       & 11            & 1,000,000  & SoftAbs Metric                    & \xmark & \cmark                                     \\
\begin{tabular}[c]{@{}l@{}}Stochastic\\ Volatility\end{tabular}     & 1000 + 3      & 100,000    & Fisher Information + Hessian      & \cmark & \cmark                                     \\
\begin{tabular}[c]{@{}l@{}}Log-Gaussian\\ Cox-Poisson\end{tabular}  & 1024 + 2      & 5,000      & Fisher Information + Hessian      & \cmark & \cmark                                     \\
Fitzhugh-Nagumo                                                     & 3             & 100,000    & Fisher Information + Hessian      & \xmark & \xmark                                     \\
\begin{tabular}[c]{@{}l@{}}Multivariate \\ Student-$t$\end{tabular} & 20            & 1,000,000  & Positive Definite Part of Hessian & \xmark & \cmark                                     \\ \bottomrule
\end{tabular}
\caption{Summary of the posterior distributions we examine in our experimental results. For the heirarchical models, we employ an alternating Metropolis-within-Gibbs-like strategy; we indicate the dimensionality of each alternating component by separating them with a plus-sign. The Neal Funnel distribution has a hierarchical structure but it is sampled in a non-hierarchical manner. As discussed in detail later, the Fitzhugh-Nagumo model computes approximate gradients by solving initial value problems.}
\label{tab:posteriors}
\end{table}
